Pointillism: Accurate 3D bounding box estimation with multi-radars

Autonomous perception requires high-quality environment sensing in the form of 3D bounding boxes of dynamic objects. The primary sensors used in automotive systems are light-based cameras and LiDARs. However, they are known to fail in adverse weather conditions. Radars can potentially solve this problem as they are barely affected by adverse weather conditions. However, specular reflections of wireless signals cause poor performance of radar point clouds. We introduce Pointillism, a system that combines data from multiple spatially separated radars with an optimal separation to mitigate these problems. We introduce a novel concept of Cross Potential Point Clouds, which uses the spatial diversity induced by multiple radars and solves the problem of noise and sparsity in radar point clouds. Furthermore, we present the design of RP-net, a novel deep learning architecture, designed explicitly for radar's sparse data distribution, to enable accurate 3D bounding box estimation. The spatial techniques designed and proposed in this paper are fundamental to radars point cloud distribution and would benefit other radar sensing applications.

==> intro-v7.tex <==
% tex 
\section{INTRODUCTION}
%Autonomous perception is a rapidly growing field these days. [some statistic here]. 
%The control system of an 

\todo{what is the problem}
Autonomous vehicles require a high-quality perception~\cite{van2018autonomous} of the scene in which they are navigating.  
Specifically, they need to perceive dynamic objects with high fidelity in 3D. The control system of
 autonomous systems expect accurate 3D bounding boxes for the dynamic objects~\cite{darms2008classification,3dperception,3dperception2} present in a scene.
 Most of the existing computer vision algorithms and data-driven techniques rely on high resolution, multi-channel LiDARs~\cite{perception,shi2018pointrcnn,wang2019frustum,Qi_2018} to construct accurate 
 3D bounding boxes for dynamic objects. Unfortunately, a LiDAR cannot penetrate through fog and dust, causing the sensor to fall prey to adverse weather conditions~\cite{dmv,bad_weather,forbes}. In contrast, radars are a robust sensing solution, which transmits millimeter waves 
 (mmWaves) and remain less affected by adverse weather conditions~\cite{lidar_radar}.
 
 %even high-resolution LiDAR's fail to sense dynamic objects in fog, or smoke or dust, causing for un-reliability of perception in all possible environmental. 
 
%A passive sensor like a camera is singularly dependent on the ambient lighting conditions and could easily fail at night or during the times of poor visibility~\cite{dmv,bad_weather,forbes}. 


%dynamic objects inside a scene in real-time. 
%Control decisions are made by combining this data with HD maps of the static environment. 



% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{images/first_image.pdf}
% \caption{Comparison of LiDAR and Radar point cloud. X marks the position of observer. The region containing a car is highlighted. Radar point clouds are much more sparse and non-uniform as compared to LiDAR. \todo{this figure, either should show same radar point clouds in good and bad weather, problem with lidar or your hardware setup, I would suggest removing it, this figure doesn't work}} 
% \label{fig:bad_weather}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/intro_fig.pdf}
\caption{ a) Single radar misses the reflective surface due to specular reflections (red). b) Multi-radar setup with optimal separation receives reflections back almost surely from the reflective surface (green). (c) Shows \name deployment in a real-world setting with overlapping FOVs of multiple radars to enable high-resolution sensing.}
\label{fig:specular}
\squeezeup
\end{figure}



\todo{In this work, we show that radars are reliant sensors for accurate 3D bounding box prediction in dynamic scenes in all weather conditions}%% stress on the detection not the all weather aspect as that is already established.
In this work, we show that radars can be used as an all-weather reliant sensor to achieve accurate 3D bounding boxes for dynamic objects. Although radars are all-weather reliant sensors, they have to provide LiDAR-like high-quality perception performance, to be considered as a primary sensing modality. However, a challenge with the radar sensor is that it cannot create dense and feature-rich point clouds for bounding box estimation. The primary reason is that an automotive radar emits mmWave signals, which tend to reflect specularly off of surfaces,
allowing only a fraction of incident waves to travel back to the sensor, as shown in Figure~\ref{fig:specular}. 
Even a high quality 1-degree angular resolution radar suffers from the curse of specularity and could not gather sufficient information from a scene for precise bounding box estimation. %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Are we showing this anywhere? Maybe we should mention that this is the case. It needs to be supported %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%A single standalone radar is not able to gather sufficient information from a scene for precise bounding box estimation. %This effect is contrary to that in LiDARs, where the nanometer level wavelength of laser beams cause them to scatter in all directions after the incidence, due to surface roughness.

\todo{be specific and how this solves the challenging problem in the previous paragraph}
In this work, we propose \name, a system that consist of multiple radars overlooking the same scene and novel multi-radar fusion algorithms to tackle the problem of specular reflections. The key idea is that multiple radars placed at spatially separated locations with optimal separation (Section \ref{sec:Multi-radar}), illuminate an object in the scene from different viewpoints. This, in turn, increases the probability of receiving a reflection back from multiple surfaces of the object, which single radars may miss, as shown in Figure~\ref{fig:specular}. This spatial diversity captures a sufficient amount of features from the objects,
making the radar data denser for use in high-quality inference. Motivated by this observation, \name builds an end-to-end multi-radar processing pipeline that enables accurate 3D bounding box estimation using multiple automotive radars.

While \name can provide rich features of the scene, precise 3D bounding box estimation still involves challenges. A critical issue is the sparsity of radar point clouds. Due to the non-uniform interaction of mmWaves with different surfaces, a radar point cloud is distributed sparsely across 3D space. Unlike LiDARs, where the point cloud distribution is fairly uniform due to the uniform scattering properties of the laser from all surfaces, one needs to account for the non-uniformity in radar point clouds to make any inference. To further exacerbate the issue, radar data contains noise due to sensor leakage, background clutter, and multi-path effects. 
This noise pollutes the point clouds by causing unwanted points to appear in the scene point cloud. 


\name presents a novel solution that jointly solves the noise and sparsity problem for efficient 3D bounding box estimation. The solution uses spatial diversity generated by multiple radar sensors to tackle noise and sparsity. A naive algorithm would be to translate the point clouds collected by each radar to a common frame of reference and combine them to densify the point cloud. However, this approach misses out on the crucial information encoded in the spatial locations of radars. We make two key observations. First, we observe that across multiple viewpoints (radars), the noise appears independent of each other. Second, the points belonging to actual surface/object appear consistently in most of the views. To best leverage the two observations, we create a space-time coherence based framework for mixing of 3D point clouds from multiple radars. This framework identifies the noise as points with a low confidence score. The output is a novel representation of \textit{\pcname} that have the information regarding the confidence of each point coming from an actual object along with all the properties of a point cloud.

% We define Log-Likelihood point clouds as an extended representation of 3D point clouds that contain the likelihood estimates for all the points.

% \todo{start new paragrph here and talk about segmentation} With log-likelihood point clouds, \ClustName can simultaneously densify the sparse point clouds by combining data from multiple radars and segment out the object point clouds by identifying noise points based on log-likelihood values. 

 

% solve the jump by telling me about segmentation and bounding boxes can have many solutions... 
% exponential solution space 
% therefore we resort to experiential learning 

With the knowledge of confidence estimates for the points, we can infer whether they belong to objects or noise. However, merely identifying all the relevant points out of noise is not sufficient for 3D bounding box estimation. Depending on the distance, orientation, and the exposed surface of an object, only a limited set of features could be captured by the radar. This results in massive uncertainty in the exact orientation and the location of the bounding box. In a scene with multiple objects, precise 3D bounding box estimation requires \todo{object based point segmentation followed by solving for uncertainty in position and orientation}first segmenting out the points belonging to each object and then solving the uncertainty present in the location and the orientation of the bounding box. However, there would be an exponentially huge solution space for a set of bounding boxes that could fit a given scene point cloud. Our insight here is that a data-driven method could potentially solve this problem by building experience over time. \todo{the rest of this is not necessary. It is repetitive}In simple words, there could be many possible placements of bounding boxes over radar generated point clouds, however, only so many of them could match to the realistic driving scenarios with the shape and sizes seen typically in the outdoor settings. To learn the exact placement of bounding boxes over radar generated point clouds, we need to combine the experiential learning with the non-uniform \pcname. 

%could be learned together with the context within a scene to estimate precise 3D bounding boxes. 

To build experiential learning, an approach could be to design hand-crafted features by taking into account the shape and size of the vehicles and all possible orientations. However, such an approach is not trivial because crafting the features that can incorporate all possible cases is very challenging. Instead, we reap the advantages of data-driven learning for precise 3D bounding box estimation and propose a novel deep learning-based approach \textit{\network}, that leverages the sparsity of \pcname. \textit{\network} combines the two problems of point cloud segmentation and 3D bounding box location estimation in space, and performs a region of interest (RoI) based classification. However, picking RoIs uniformly throughout the 3D space is not computationally feasible. So, we define a unique set of anchor boxes that allow us to iterate over all the possible configurations of bounding boxes over sparse point clouds. Further, our experiments show that with this set of anchor boxes, we can exhaustively cover all the configurations while efficiently reducing the search space. Our solution is an end-to-end trainable network, which can easily be deployed for real-life testing.
 

It is well known that a data-driven approach needs a lot of data for training and validation. To the best of our knowledge, there is only three publicly available datasets for automotive radars, the NuScenes dataset~\cite{nuscenes2019}, Oxford Mechanical radar~\cite{RadarRobotCarDatasetArXiv} and Astyx HiRes~\cite{astyx}, however, none of them contains data from multiple radars with overlapping field of views. Due to the lack of data, we built an automated data collection platform with multiple radars along with a LiDAR and a depth camera for ground truth labels.
 To prototype \name's design, we created a first of its kind dataset of \datasize radar frames from real-world radar scans in diverse automotive scenarios, including good/bad weather, and manually labeled the data over a period of two months\footnote{We would release our dataset for the benefit of the research community.}. We use this dataset for training and testing our network. 

% \name achieves an overall mAP score of \textbf{0.67} with an IoU threshold of 0.5 for estimating 3D bounding box. This is a \textbf{35\%} improvement over the performance achieved by a single radar. 

% of bounding boxes of objects within a median error of less than \textbf{xxcm} and estimate the dimensions of the box within a median error of \textbf{xxcm} over xm. 
\name achieves an overall mAP score~\cite{Geiger2012CVPR} of \textbf{0.67} with an IoU threshold of 0.5 and \textbf{0.94} with an IoU threshold of 0.2 for estimating 3D bounding box, which is comparable with the state-of-the-art bounding box estimation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% should we name the techniques? %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
techniques~\cite{Qi_2018,shi2018pointrcnn,shi2019pv} using LiDARs. Furthermore, with our approach, the mAP values increase to \textbf{0.67} compared to \textbf{0.45} for a single radar system. This means that \name improves the performance by \textbf{48\%} with its multi-radar fusion compared to a single radar.

In summary, our contributions are as follows:
\vspace{-0.08in}
\begin{itemize}
    % \setlength\itemsep{-0em}
    \item We propose \name, a new framework for radar perception that uses multiple radars placed at spatially separated locations, to counter the fundamental challenge of specular reflections in mmWave radars.
    \item We conceptualize the notion of \textit{\pcname} by utilizing space-time coherence on point clouds from multiple radars, to solve the problem of radar point cloud sparsity and noise.
    \item We provide the design of \textit{\network}, a novel deep learning framework, designed to leverage the non-uniform distribution of radar point clouds, and estimate precise 3D bounding boxes on \pcname.
    \item We build the first real-world dataset of labeled radar point clouds from multiple radars with overlapping field of view, that contains \datasize radar frames and corresponding LiDAR point clouds and RGB images. We believe that this dataset would enable innovation in a variety of sensor-fusion approaches.
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 

% \todo{KESHAV's COMMENT: we did not use Lidar in the dataset, we should not claim that. When you release it and there is no lidar people will be mad. Also a lot of the bootom paragraph is redundant as it was summarized above.}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  Finally, we would release the real-world data-set collected with \name's radar, LiDar and intel real sense for larger community to make this reality in near future. 
